Error Correcting Codes for Distributed Control

The problem of stabilizing an unstable plant over a noisy communication link is an increasingly important one that arises in applications of networked control systems. Although the work of Schulman and Sahai over the past two decades, and their development of the notions of "tree codes"\phantom{} and "anytime capacity", provides the theoretical framework for studying such problems, there has been scant practical progress in this area because explicit constructions of tree codes with efficient encoding and decoding did not exist. To stabilize an unstable plant driven by bounded noise over a noisy channel one needs real-time encoding and real-time decoding and a reliability which increases exponentially with decoding delay, which is what tree codes guarantee. We prove that linear tree codes occur with high probability and, for erasure channels, give an explicit construction with an expected decoding complexity that is constant per time instant. We give novel sufficient conditions on the rate and reliability required of the tree codes to stabilize vector plants and argue that they are asymptotically tight. This work takes an important step towards controlling plants over noisy channels, and we demonstrate the efficacy of the method through several examples.

==> DecodingBEC.tex <==
\section{Decoding over the Binary Erasure Channel}
\label{sec: DecodingBEC}

Owing to the simplicity of the erasure channel, it is possible to come up with an efficient way to perform maximum likelihood decoding at each time step. We will show that the average complexity of the decoding operation at any time $t$ is constant and that it being larger than $KC^3$ decays exponentially in $C$. Consider an arbitrary decoding instant $t$, let $c=[c_1^T,\ldots,c_t^T]^T$ be the transmitted codeword and let $z=[z_1^T,\ldots,z_t^T]^T$ denote the corresponding channel outputs. Recall that $\mathbb{H}_{n,R}^t$ denotes the $\overline{n}t\times nt$ leading principal minor of $\mathbb{H}_{n,R}$. Let $z_e$ denote the erasures in $z$ and let $H_e$ denote the columns of $\mathbb{H}_{n,R}^t$  that correspond to the positions of the erasures. Also, let $\tilde{z}_e$ denote the unerased entries of $z$ and let $\tilde{H}_e$ denote the columns of $\mathbb{H}_{n,R}^t$ excluding $H_e$. So, we have the following parity check condition on $z_e$, $H_ez_e = \tilde{H}_e\tilde{z}_e$. Since $\tilde{z}_e$ is known at the decoder, $s\triangleq \tilde{H}_e\tilde{z}_e$ is known. Maximum likelihood decoding boils down to solving the linear equation $H_ez_e = s$. Due to the lower triangular nature of $H_e$, unlike in the case of traditional block coding, this equation will typically not have a unique solution, since $H_e$ will typically not have full column rank. This is alright as we are not interested in decoding the entire $z_e$ correctly, we only care about decoding the earlier entries accurately. If $z_e = [z_{e,1}^T,\,\, z_{e,2}^T]^T$, then $z_{e,1}$ corresponds to the earlier time instants while $z_{e,2}$ corresponds to the latter time instants. The desired reliability requires one to recover $z_{e,1}$ with an exponentially smaller error probability than $z_{e,2}$. Since $H_e$ is lower triangular, we can write $H_ez_e = s$ as%\eqref{eq: ml} as
\begin{align}
\label{eq: bec1}
 \left[\begin{array}{cc}
  H_{e,11} & 0\\
  H_{e,21} & H_{e,22}
 \end{array}\right]\left[\begin{array}{c}z_{e,1}\\z_{e,2}\end{array}\right] = \left[\begin{array}{c}s_1\\s_2\end{array}\right]
\end{align}
Let $H_{e,22}^\bot$ denote the orthogonal complement of $H_{e,22}$, ie., $H_{e,22}^\bot H_{e,22} = 0$. Then multiplying both sides of \eqref{eq: bec1} with diag$(I,H_{e,22})$, we get
\begin{align}
 \label{eq: bec2}
 \left[\begin{array}{c}
  H_{e,11}\\
  H_{e,22}^\bot H_{e,21}
 \end{array}\right]z_{e,1} = \left[\begin{array}{c}s_1\\H_{e,22}^\bot s_2\end{array}\right]
\end{align}
If $[H_{e,11}^T\,\,\, (H_{e,22}^\bot H_{e,21})^T]^T$ has full column rank, then $z_{e,1}$ can be recovered exactly. The decoding algorithm now suggests itself, i.e., find the smallest possible $H_{e,22}$ such that $[H_{e,11}^T\,\,\, (H_{e,22}^\bot H_{e,21})^T]^T$ has full rank and it is outlined in Algorithm \ref{alg: algorithm}.
\begin{algorithm}
\caption{Decoder for the BEC}
\label{alg: algorithm}
\begin{enumerate}
\item Suppose, at time $t$, the earliest uncorrected error is at a delay $d$. Identify $z_e$ and $H_e$ as defined above.
\item Starting with $d'=1,2,\ldots,d$, partition
\begin{align*}
 z_e = [z_{e,1}^T\,\,z_{e,2}^T]^T\,\,\text{and}\,\,H_e = \left[\begin{array}{cc}H_{e,11}&0\\H_{e,21}&H_{e,22}\end{array}\right]
\end{align*}
where $z_{e,2}$ correspond to the erased positions up to delay $d'$.
\item Check whether the matrix $\left[\begin{array}{c}
  H_{e,11}\\
  H_{e,22}^\bot H_{e,21}
 \end{array}\right]$
% \begin{align*}
%  \left[\begin{array}{c}
%   H_{e,11}\\
%   H_{e,22}^\bot H_{e,21}
%  \end{array}\right]
% \end{align*}
has full column rank.
\item If so, solve for $z_{e,1}$ in the system of equations
\begin{align*}
  \left[\begin{array}{c}
  H_{e,11}\\
  H_{e,22}^\bot H_{e,21}
 \end{array}\right]z_{e,1} = \left[\begin{array}{c}s_1\\H_{e,22}^\bot s_2\end{array}\right]
\end{align*}
\item Increment $t=t+1$ and continue.
\end{enumerate}
\end{algorithm} 

\subsection{Complexity}
Suppose the earliest uncorrected error is at time $t-d+1$, then steps 2), 3) and 4) in Algorithm \ref{alg: algorithm} can be accomplished by just reducing $H_e$ into the appropriate row echelon form, which has complexity $\OO{d^3}$. The earliest entry in $z_e$ is at time $t-d+1$ implies that it was not corrected at time $t-1$, the probability of which is $P_{d-1,t-1}^e \leq \eta 2^{-n\beta (d-1)}$. Hence, the average decoding complexity is at most $K\sum_{d>0}d^3 2^{-n\beta d}$ which is bounded and is independent of $t$. In particular, the probability of the decoding complexity being $Kd^3$ is at most $\eta 2^{-n\beta d}$. The decoder is easy to implement and its performance is simulated in Section \ref{sec: Simulations}. Note that the encoding complexity per time iteration increases linearly with time. This can also be made constant on average if the decoder can send periodic acks back to the encoder with the time index of the last correctly decoded source bit. 

\subsection{Extension to Packet Erasures}
The encoding and decoding algorithms presented so far have been developed for the case of bit erasures. But it is not difficult to see that the techniques generalize to the case of packet erasures. For example, for a packet length $L$, what was one bit earlier will now be a block of $L$ bits. Each binary entry in the encoding/parity check matrix will now be an $L\times L$ binary matrix. The rate will remain the same. So, at each time, $k$ packets each of length $L$  will be encoded to $n$ packets each of the same length $L$. Recall that the \textit{anytime performance} of the code is determined by the delay dependent codebook $\mathcal{C}_{t,d}$ and its distance distribution $\{\numW{w}{d}{t}\}_{w=1}^{nd}$. In the case of packet erasures, one can obtain analogous results by defining the Hamming distance of a codeword slightly differently. By viewing a codeword as a collection of packets, define its Hamming distance to be the number of non zero packets. The definition of the delay dependent distance distribution $\{\numW{w}{d}{t}\}$ will change accordingly. With this modification, one can easily apply the results developed in Sections \ref{sec: Sufficient Condition}, \ref{sec: Existence} and the decoding algrithm in Section \ref{sec: DecodingBEC} above to the case of packet erasures.

==> RecapOfBlockCodes.tex <==
\section{A Brief Recap of Random Coding}

For an arbitrary discrete memoryless channel, recall the following familiar definition of the random coding exponent $E_r(R)$ from \cite{Gallager}\footnote{We use base-2 instead of the natural logarithm}
\begin{subequations}
\begin{align}
\label{eq: randomCodingExponent}E_r(R) &= \max_{0\leq\rho\leq 1}\max_{\mathbf{Q}}\left[E_o\bra{\rho,\mathbf{Q}}-\rho R\right],\,\,\text{where}\\
 E_o\bra{\rho,\mathbf{Q}} &= -\log_2\sum_{z\in\mathcal{Z}}\left[\sum_{x\in\mathcal{X}}Q(x)p(z|X=x)^{\frac{1}{1+\rho}}\right]^{1+\rho}
\end{align}
\end{subequations}
$E_r(R)$ is the Gallager's random coding exponent. For a linear code with block length $m$, let $\{N_w\}_{w=1}^N$ denote its distance distribution, i.e., $N_w$ is the number of codewords with Hamming weight $w$. Then, we have the following result
\begin{lem}
Consider a linear code with block length $m$, rate $R$ and distance distribution $\{N_w\}_{w=1}^N$ such that
\begin{enumerate}
 \item $N_w = 0$ if $w \leq H^{-1}(1-R-\delta)$
 \item $N_w \leq 2^{-m(1-R-\delta+o(1))}\binom{m}{w}$
\end{enumerate}
for some $\delta > 0$. Let the channel be a binary input ouput symmetric channel with Bhattacharya parameter $\bh$. Then the block error probability, $P_e$, under ML decoding is bounded as
\begin{align}
 P_e \leq 2^{-m\bra{E_\bh(R) - \delta'}}
\end{align}
where 
\begin{align}
 E_\bh(R) = \left\{\begin{array}{cc}
                    H^{-1}(1-R)\log\frac{1}{\bh} & ,\,\,\,0\leq R\leq 1 - H\bra{\frac{\bh}{1+\bh}}\\
		    E_r(R)            & ,\,\,\, 1 - H\bra{\frac{\bh}{1+\bh}}\leq R\leq C
                   \end{array}
		\right.
\end{align}
and $\delta'\rightarrow 0$ as $\delta\rightarrow 0$.
\end{lem}
\begin{IEEEproof}
 The proof is a straightforward generalization of the result in \cite{Barg}.
\end{IEEEproof}

